FCBench: Cross-Domain Benchmarking of Lossless Compression for Floating-Point Data

While both the database and high-performance computing (HPC) communities utilize lossless compression methods to minimize floating-point data size, a disconnect persists between them. Each community designs and assesses methods in a domain-specific manner, making it unclear if HPC compression techniques can benefit database applications or vice versa. With the HPC community increasingly leaning towards in-situ analysis and visualization, more floating-point data from scientific simulations are being stored in databases like Key-Value Stores and queried using in-memory retrieval paradigms. This trend underscores the urgent need for a collective study of these compression methods' strengths and limitations, not only based on their performance in compressing data from various domains but also on their runtime characteristics. Our study extensively evaluates the performance of eight CPU-based and five GPU-based compression methods developed by both communities, using 33 real-world datasets assembled in the Floating-point Compressor Benchmark (FCBench). Additionally, we utilize the roofline model to profile their runtime bottlenecks. Our goal is to offer insights into these compression methods that could assist researchers in selecting existing methods or developing new ones for integrated database and HPC applications.

==> tables/comp_ratio.tex <==
\begin{tabular}{@{} llrrrrrrrrr|rrrrr @{}}
       \toprule
       \bfseries Name         & \bfseries Domain  & \bfseries pFPC      & \bfseries SPDP    & \bfseries fpzip
                              & \bfseries shf+LZ4 & \bfseries shf+zstd  & \bfseries ndzip-C
                              & \bfseries BUFF    & \bfseries Gorilla   & \bfseries Chimp
                              & \bfseries GFC     & \bfseries MPC
                              & \bfseries nv::LZ4 & \bfseries nv::btcmp
                              & \bfseries ndzip-G
       \\
       \midrule
       \textbf{msg-bt}        & HPC               & 1.25                & 1.33              & 1.20            & 1.21  & 1.19          & 1.13  & 1.02 & 1.09  & 1.13 & 1.09 & 1.15          & 1.06  & 1.21  & 1.13  \\
       \textbf{num-brain}     & HPC               & 1.15                & 1.20              & 1.25            & 1.17  & 1.18          & 1.16  & 1.94 & 1.11  & 1.17 & 1.09 & 1.18          & 1.00  & 1.17  & 1.16  \\
       \textbf{num-control}   & HPC               & 1.04                & 1.01              & 1.12            & 1.11  & 1.12          & 1.11  & 2.00 & 0.98  & 1.06 & 1.01 & 1.11          & 1.01  & 1.11  & 1.11  \\
       \textbf{rsim}          & HPC               & 1.35                & 1.69              & 1.48            & 1.50  & 1.56          & 1.97  & 0.60 & 1.34  & 1.34 & 1.30 & 1.53          & 1.31  & 1.50  & 1.97  \\
       \textbf{astro-mhd}     & HPC               & 10.93               & 20.93             & 30.3            & 12.37 & 17.51         & 12.58 & 1.42 & 18.60 & 5.97 & \NA  & 8.35          & 22.82 & 20.80 & 12.58 \\
       \textbf{astro-pt}      & HPC               & 1.28                & 1.40              & 1.32            & 1.20  & 1.21          & 1.42  & 1.83 & 1.03  & 1.22 & \NA  & 1.26          & 1.00  & 1.00  & 1.42  \\
       \textbf{miranda3d}     & HPC               & 1.14                & 1.19              & 2.20            & \NA   & \NA           & 1.83  & 0.97 & 1.04  & 1.18 & \NA  & 1.60          & 1.02  & 1.02  & \NA   \\
       \textbf{turbulence}    & HPC               & 1.01                & 1.05              & 1.31            & 1.15  & 1.16          & 1.23  & 0.82 & 0.99  & 1.02 & 1.00 & 1.21          & 1.00  & 1.15  & 1.23  \\
       \textbf{wave}          & HPC               & 1.16                & 1.90              & 1.58            & 1.29  & 1.31          & 1.99  & 1.00 & 1.03  & 1.15 & 1.02 & 1.52          & 1.03  & 1.29  & 1.99  \\
       \textbf{hurricane}     & HPC               & 0.95                & 1.37              & 0.99            & 1.51  & 1.55          & 0.99  & \NA  & 1.06  & 0.99 & 0.94 & 1.54          & 1.00  & 1.00  & 0.99  \\
       \midrule
       \textbf{citytemp}      & TS                & 1.08                & 1.01              & 1.47            & 2.24  & 2.31          & 1.31  & 0.82 & 1.03  & 1.26 & 1.08 & 1.35          & 1.37  & 1.01  & 1.31  \\
       \textbf{ts-gas}        & TS                & 1.34                & 1.41              & 1.93            & 1.43  & 1.50          & 1.47  & 0.67 & 1.20  & 1.45 & 1.17 & 1.51          & 1.56  & 1.43  & 1.47  \\
       \textbf{phone-gyro}    & TS                & 1.34                & 1.41              & 1.93            & 1.43  & 1.50          & 1.47  & 0.67 & 1.20  & 1.45 & 1.17 & 1.51          & 1.56  & 1.43  & 1.47  \\
       \textbf{wesad-chest}   & TS                & 1.34                & 1.41              & 1.93            & 1.43  & 1.50          & 1.47  & 0.67 & 1.20  & 1.45 & 1.17 & 1.51          & 1.56  & 1.43  & 1.47  \\
       \textbf{jane-street}   & TS                & 1.34                & 1.41              & 1.93            & 1.43  & 1.50          & 1.47  & 0.67 & 1.20  & 1.45 & 1.17 & 1.51          & 1.56  & 1.43  & 1.47  \\
       \textbf{nyc-taxi}      & TS                & 1.34                & 1.41              & 1.93            & 1.43  & 1.50          & 1.47  & 0.67 & 1.20  & 1.45 & 1.17 & 1.51          & 1.56  & 1.43  & 1.47  \\
       \textbf{gas-price}     & TS                & 1.34                & 1.41              & 1.93            & 1.43  & 1.50          & 1.47  & 0.67 & 1.20  & 1.45 & 1.17 & 1.51          & 1.56  & 1.43  & 1.47  \\
       \textbf{solar-wind}    & TS                & 1.34                & 1.41              & 1.93            & 1.43  & 1.50          & 1.47  & 0.67 & 1.20  & 1.45 & 1.17 & 1.51          & 1.56  & 1.43  & 1.47  \\
       \midrule
       \textbf{acs-wht}       & OBS               & 0.94                & 1.00              & 0.99            & 1.00  & 1.00          & 0.98  & \NA  & 0.97  & 0.97 & 0.94 & 0.97          & 1.00  & 1.00  & 0.98  \\
       \textbf{hdr-night}     & OBS               & 0.94                & 1.00              & 0.99            & 1.00  & 1.00          & 0.98  & \NA  & 0.97  & 0.97 & 0.94 & 0.97          & 1.00  & 1.00  & 0.98  \\
       \textbf{hdr-lalermo}   & OBS               & 0.94                & 1.00              & 0.99            & 1.00  & 1.00          & 0.98  & \NA  & 0.97  & 0.97 & 0.94 & 0.97          & 1.00  & 1.00  & 0.98  \\
       \textbf{hst-wfc3-uvis} & OBS               & 0.94                & 1.00              & 0.99            & 1.00  & 1.00          & 0.98  & \NA  & 0.97  & 0.97 & 0.94 & 0.97          & 1.00  & 1.00  & 0.98  \\
       \textbf{hst-wfc3-ir}   & OBS               & 0.94                & 1.00              & 0.99            & 1.00  & 1.00          & 0.98  & \NA  & 0.97  & 0.97 & 0.94 & 0.97          & 1.00  & 1.00  & 0.98  \\
       \textbf{spitzer-irac}  & OBS               & 1.15                & 1.23              & 1.17            & 1.36  & 1.38          & 1.19  & \NA  & 1.85  & 1.77 & 1.15 & 1.34          & 1.23  & 1.36  & 1.19  \\
       \textbf{g24-78-usb}    & OBS               & 0.94                & 1.00              & 0.99            & 1.00  & 1.00          & 0.98  & \NA  & 0.97  & 0.97 & 0.94 & 0.97          & 1.00  & 1.00  & 0.98  \\
       \textbf{jws-mirimage}  & OBS               & 0.94                & 1.00              & 0.99            & 1.00  & 1.00          & 0.98  & \NA  & 0.97  & 0.97 & 0.94 & 0.97          & 1.00  & 1.00  & 0.98  \\
       \midrule
       \textbf{tpcH-order}    & DB                & 1.02                & 1.02              & 1.17            & 1.30  & 1.30          & 1.10  & 1.25 & 1.08  & 1.58 & 1.07 & 1.12          & 1.50  & 1.30  & 1.10  \\
       \textbf{tpcxBB-store}  & DB                & 1.02                & 1.02              & 1.17            & 1.30  & 1.30          & 1.10  & 1.25 & 1.08  & 1.58 & 1.07 & 1.12          & 1.50  & 1.30  & 1.10  \\
       \textbf{tpcxBB-web}    & DB                & 1.02                & 1.02              & 1.17            & 1.30  & 1.30          & 1.10  & 1.25 & 1.08  & 1.58 & 1.07 & 1.12          & 1.50  & 1.30  & 1.10  \\
       \textbf{tpcH-lineitem} & DB                & 1.02                & 1.02              & 1.13            & 1.33  & 1.46          & 0.98  & 0.67 & 0.98  & 1.62 & \NA  & 1.01          & 1.51  & 1.33  & 0.98  \\
       \textbf{tpcDS-catalog} & DB                & 1.02                & 1.02              & 1.17            & 1.30  & 1.30          & 1.10  & 1.25 & 1.08  & 1.58 & 1.07 & 1.12          & 1.50  & 1.30  & 1.10  \\
       \textbf{tpcDS-store}   & DB                & 1.02                & 1.02              & 1.17            & 1.30  & 1.30          & 1.10  & 1.25 & 1.08  & 1.58 & 1.07 & 1.12          & 1.50  & 1.30  & 1.10  \\
       \textbf{tpcDS-web}     & DB                & 1.02                & 1.02              & 1.17            & 1.30  & 1.30          & 1.10  & 1.25 & 1.08  & 1.58 & 1.07 & 1.12          & 1.50  & 1.30  & 1.10  \\



       \hline
       \textbf{harmonic mean} & -                 & 1.18                & 1.28              & 1.37            & 1.38  & \textbf{1.41} & 1.33  & 1.16 & 1.16  & 1.28 & 1.06 & \textbf{1.33} & 1.21  & 1.11  & 1.30  \\
       \bottomrule
\end{tabular}

==> tables/comp_speed.tex <==
\begin{tabular}{@{} llrrrrrrrrr|rrrrr @{}}
        \toprule
        \bfseries Name           & \bfseries Domain  & \bfseries pFPC      & \bfseries SPDP    & \bfseries fpzip
                                 & \bfseries shf+LZ4 & \bfseries shf+zstd  & \bfseries ndzip-C
                                 & \bfseries BUFF    & \bfseries Gorilla   & \bfseries Chimp
                                 & \bfseries GFC     & \bfseries MPC
                                 & \bfseries nv::LZ4 & \bfseries nv::btcmp
                                 & \bfseries ndzip-G
        \\
        \midrule
        \textbf{msg-bt}          & HPC               & 23.391              & 0.200             & 0.079           & 0.733 & 1.124 & 2.523 & 0.216 & 0.041 & 0.034 & 87.728  & 28.386 & 1.670  & 203.539          & 81.450  \\
        \textbf{num-brain}       & HPC               & 23.720              & 0.183             & 0.077           & 0.627 & 1.238 & 2.251 & 0.306 & 0.038 & 0.031 & 113.012 & 27.950 & 1.548  & 247.459          & 79.867  \\
        \textbf{num-control}     & HPC               & 23.232              & 0.159             & 0.073           & 0.746 & 1.168 & 2.392 & 0.309 & 0.040 & 0.032 & 75.830  & 27.490 & 1.576  & 248.455          & 78.515  \\
        \textbf{rsim}            & HPC               & 18.854              & 0.217             & 0.070           & 0.499 & 1.328 & 2.981 & 0.128 & 0.041 & 0.038 & 85.500  & 30.411 & 2.023  & 235.651          & 84.430  \\
        \textbf{astro-mhd}       & HPC               & 19.247              & 0.447             & 0.317           & 1.902 & 3.270 & 8.419 & 0.271 & 0.199 & 0.074 & N/A     & 28.459 & 27.359 & 287.823          & 174.869 \\
        \textbf{astro-pt}        & HPC               & 23.103              & 0.203             & 0.094           & 1.150 & 1.231 & 3.464 & 0.403 & 0.038 & 0.030 & N/A     & 28.345 & 1.580  & 256.929          & 67.832  \\
        \textbf{miranda3d}       & HPC               & 26.597              & 0.155             & 0.080           & N/A   & N/A   & 4.381 & 0.154 & 0.028 & 0.031 & N/A     & 34.710 & 1.647  & 261.586          & N/A     \\
        \textbf{turbulence}      & HPC               & 22.595              & 0.145             & 0.063           & 0.489 & 0.990 & 1.825 & 0.145 & 0.027 & 0.034 & 73.444  & 30.805 & 1.473  & 235.055          & 66.419  \\
        \textbf{wave}            & HPC               & 25.121              & 0.217             & 0.112           & 1.104 & 1.272 & 4.683 & 0.139 & 0.034 & 0.033 & 103.520 & 30.712 & 1.460  & 256.988          & 75.999  \\
        \textbf{hurricane}       & HPC               & 24.200              & 0.174             & N/A             & 0.495 & 1.419 & 1.488 & N/A   & 0.046 & 0.028 & 93.979  & 30.424 & 1.809  & 243.778          & 67.586  \\
        \midrule
        \textbf{citytemp}        & TS                & 9.374               & 0.109             & 0.053           & 0.141 & 1.118 & 0.741 & 0.142 & 0.045 & 0.027 & 88.142  & 28.176 & 0.475  & 144.801          & 56.984  \\
        \textbf{ts-gas}          & TS                & 20.248              & 0.186             & 0.071           & 0.922 & 1.403 & 3.080 & 0.118 & 0.033 & 0.034 & 90.527  & 30.670 & 2.034  & 248.964          & 81.300  \\
        \textbf{phone-gyro}      & TS                & 25.762              & 0.173             & 0.075           & 0.869 & 1.281 & 0.967 & 0.297 & 0.040 & 0.037 & 71.971  & 28.664 & 1.694  & 253.557          & 261.696 \\
        \textbf{wesad-chest}     & TS                & 24.956              & 0.256             & 0.079           & 1.043 & 2.052 & 0.966 & 0.301 & 0.053 & 0.029 & 73.710  & 27.887 & 3.221  & 253.955          & 261.480 \\
        \textbf{jane-street}     & TS                & 26.521              & 0.157             & 0.075           & 1.153 & 0.955 & 1.984 & 0.367 & 0.040 & 0.032 & N/A     & 29.331 & 1.616  & 259.426          & 81.645  \\
        \textbf{nyc-taxi}        & TS                & 27.213              & 0.129             & 0.081           & 1.198 & 1.414 & 1.027 & 0.241 & 0.049 & 0.030 & N/A     & 28.211 & 3.170  & 219.355          & 262.811 \\
        \textbf{gas-price}       & TS                & 24.043              & 0.165             & 0.082           & 1.239 & 1.265 & 1.042 & 0.309 & 0.036 & 0.044 & N/A     & 28.389 & 3.881  & 257.897          & 263.055 \\
        \textbf{solar-wind}      & TS                & 26.151              & 0.165             & 0.061           & 0.916 & 1.158 & 1.016 & 0.117 & 0.043 & 0.027 & 76.956  & 29.637 & 1.064  & 254.227          & 260.294 \\
        \midrule
        \textbf{acs-wht}         & OBS               & 25.708              & 0.178             & 0.068           & 0.897 & 1.278 & 3.084 & 0.128 & 0.045 & 0.036 & 119.537 & 30.141 & 1.847  & 236.824          & 79.646  \\
        \textbf{hdr-night}       & OBS               & 25.088              & 0.206             & 0.058           & 1.406 & 2.246 & 2.715 & 0.117 & 0.044 & 0.026 & 88.921  & 30.728 & 2.346  & 214.969          & 72.254  \\
        \textbf{hdr-lalermo}     & OBS               & 26.077              & 0.215             & 0.068           & 1.755 & 2.525 & 3.208 & 0.191 & 0.051 & 0.027 & N/A     & 30.792 & 2.784  & 244.880          & 74.755  \\
        \textbf{hst-wfc3-uvis}   & OBS               & 23.095              & 0.198             & 0.076           & 0.611 & 1.384 & 2.469 & 0.137 & 0.061 & 0.044 & 84.679  & 29.523 & 2.187  & 213.712          & 94.281  \\
        \textbf{hst-wfc3-ir}     & OBS               & 14.371              & 0.165             & 0.075           & 0.252 & 1.240 & 1.014 & 0.133 & 0.043 & 0.043 & 92.819  & 29.022 & 2.164  & 148.971          & 77.675  \\
        \textbf{spitzer-irac}    & OBS               & 24.392              & 0.189             & 0.066           & 0.720 & 1.213 & 2.564 & 0.137 & 0.049 & 0.039 & 78.357  & 30.574 & 1.916  & 223.544          & 80.831  \\
        \textbf{g24-78-usb}      & OBS               & 26.800              & 0.161             & 0.060           & 1.152 & 1.013 & 2.404 & 0.201 & 0.040 & 0.035 & N/A     & 30.912 & 1.548  & 260.501          & 69.587  \\
        \textbf{jws-mirimage}    & OBS               & 23.612              & 0.153             & 0.062           & 0.680 & 1.281 & 1.796 & 0.123 & 0.031 & 0.033 & 105.544 & 30.027 & 1.625  & 250.369          & 80.921  \\
        \midrule
        \textbf{tpcH-order}      & DB                & 22.668              & 0.159             & 0.073           & 0.623 & 1.328 & 2.090 & 0.327 & 0.044 & 0.029 & 109.567 & 27.772 & 1.519  & 244.177          & 77.773  \\
        \textbf{tpcxBB-store}    & DB                & 25.491              & 0.180             & 0.075           & 1.285 & 1.478 & 1.030 & 0.256 & 0.045 & 0.035 & N/A     & 27.413 & 2.810  & 257.849          & 262.928 \\
        \textbf{tpcxBB-web}      & DB                & 25.848              & 0.177             & 0.074           & 1.322 & 1.367 & 1.033 & 0.241 & 0.043 & 0.034 & N/A     & 28.818 & 2.661  & 261.673          & 263.328 \\
        \textbf{tpcH-lineitem}   & DB                & 25.988              & 0.128             & 0.065           & 1.202 & 1.238 & 1.029 & 0.113 & 0.039 & 0.030 & N/A     & 30.470 & 2.092  & 259.098          & 262.053 \\
        \textbf{tpcDS-catalog}   & DB                & 24.202              & 0.139             & 0.057           & 0.664 & 1.161 & 0.912 & 0.132 & 0.044 & 0.028 & 72.592  & 30.446 & 1.578  & 249.906          & 255.454 \\
        \textbf{tpcDS-store}     & DB                & 26.174              & 0.147             & 0.057           & 0.822 & 1.171 & 0.969 & 0.130 & 0.047 & 0.028 & 75.454  & 30.982 & 1.788  & 253.698          & 259.086 \\
        \textbf{tpcDS-web}       & DB                & 21.722              & 0.136             & 0.057           & N/A   & N/A   & 0.792 & 0.133 & 0.044 & 0.028 & 69.331  & 30.370 & 1.465  & 239.637          & 247.518 \\
        \hline
        \textbf{arithmetic mean} & -                 & \textbf{23.502}     & 0.181             & 0.079           & 0.923 & 1.407 & 2.192 & 0.202 & 0.047 & 0.034 & 87.778  & 29.595 & 2.716  & \textbf{240.280} & 142.635 \\
        \bottomrule
\end{tabular}

==> tables/comp_speed_new.tex <==
\begin{tabu}{@{} r | rrrrrrrrr|rrrrr | @{}}
        \rowfont{\bfseries}
        \multicolumn{1}{r}{\begin{tabular}{@{}r@{}}\fontfamily{ugq}\selectfont %\normalsize 
        COMPRESSION\end{tabular}}   & 
        \TableHead{pFPC}    & 
        \TableHead{SPDP}    & 
        \TableHead{fpzip}   & 
        \TableHead{\TwoLineTabTitle{shf+}{LZ4}}   & 
        \TableHead{\TwoLineTabTitle{shf+}{zstd}}  & 
        \TableHead{\TwoLineTabTitle{ndzip}{-CPU}} & 
        \TableHead{BUFF}     & 
        \TableHead{Gorilla}  & 
        \TableHead{Chimp}    & 
        \TableHead{GFC}      & 
        \TableHead{MPC}      & 
        \TableHead{\TwoLineTabTitle{nv::}{LZ4}}   & 
        \TableHead{\TwoLineTabTitle{nv::}{btcmp}} & 
        \TableHead{\TwoLineTabTitle{ndzip}{-GPU}} 
        \\

        \cline{2-15}
        \textbf{arithmetic mean} & 0.564               & 0.181             & 0.079           & 0.923 & 1.407 & \textbf{2.192} & 0.202 & 0.047 & 0.034 & 87.778  & 29.595 & 2.716  & \textbf{240.280} & 142.635 \\
        \cline{2-15}
        % \multicolumn{1}{c}{}\\
        % \multicolumn{1}{c}{}\\
                \rowfont{\bfseries}
        \multicolumn{1}{r}{\begin{tabular}{@{}r@{}}\fontfamily{ugq}\selectfont %\normalsize 
        DECOMPRESSION
        % \\domain \& name
        \end{tabular}}   & 
        \\
        \cline{2-15}
        \textbf{arithmetic mean} & 0.351               & 0.178             & 0.074           & 1.181 & 1.328 & \textbf{1.636} & 0.254 & 0.146 & 0.175 & 99.258 & 28.513 & 53.352 & 122.483 & \textbf{159.312} \\
        \cline{2-15}
        % \bottomrule
\end{tabu}

==> tables/comp_speed_new_bkp.tex <==
\begin{tabu}{@{} r | rrrrrrrrr|rrrrr | @{}}
        \rowfont{\bfseries}
        \multicolumn{1}{r}{\begin{tabular}{@{}r@{}}\fontfamily{ugq}\selectfont %\normalsize 
        COMPRESSION\\domain \& name\end{tabular}}   & 
        % {domain} & 
        \TableHead{pFPC}    & 
        \TableHead{SPDP}    & 
        \TableHead{fpzip}   & 
        \TableHead{\TwoLineTabTitle{shf+}{LZ4}}   & 
        \TableHead{\TwoLineTabTitle{shf+}{zstd}}  & 
        \TableHead{\TwoLineTabTitle{ndzip}{-CPU}} & 
        \TableHead{BUFF}     & 
        \TableHead{Gorilla}  & 
        \TableHead{Chimp}    & 
        \TableHead{GFC}      & 
        \TableHead{MPC}      & 
        \TableHead{\TwoLineTabTitle{nv::}{LZ4}}   & 
        \TableHead{\TwoLineTabTitle{nv::}{btcmp}} & 
        \TableHead{\TwoLineTabTitle{ndzip}{-GPU}} 
        \\
        \cline{2-15}
        \NameDomain{msg-bt}{HPC}               & 0.721               & 0.200             & 0.079           & 0.733 & 1.124 & 2.523          & 0.216 & 0.041 & 0.034 & 87.728  & 28.386 & 1.670  & 203.539          & 81.450  \\
        \NameDomain{num-brain}{HPC}               & 0.577               & 0.183             & 0.077           & 0.627 & 1.238 & 2.251          & 0.306 & 0.038 & 0.031 & 113.012 & 27.950 & 1.548  & 247.459          & 79.867  \\
        \NameDomain{num-control}{HPC}               & 0.564               & 0.159             & 0.073           & 0.746 & 1.168 & 2.392          & 0.309 & 0.040 & 0.032 & 75.830  & 27.490 & 1.576  & 248.455          & 78.515  \\
        \NameDomain{rsim}{HPC}               & 0.540               & 0.217             & 0.070           & 0.499 & 1.328 & 2.981          & 0.128 & 0.041 & 0.038 & 85.500  & 30.411 & 2.023  & 235.651          & 84.430  \\
        \NameDomain{astro-mhd}{HPC}               & 1.359               & 0.447             & 0.317           & 1.902 & 3.270 & 8.419          & 0.271 & 0.199 & 0.074 & \NA     & 28.459 & 27.359 & 287.823          & 174.869 \\
        \NameDomain{astro-pt}{HPC}               & 0.885               & 0.203             & 0.094           & 1.150 & 1.231 & 3.464          & 0.403 & 0.038 & 0.030 & \NA     & 28.345 & 1.580  & 256.929          & 67.832  \\
        \NameDomain{miranda3d}{HPC}               & 0.759               & 0.155             & 0.080           & \NA   & \NA   & 4.381          & 0.154 & 0.028 & 0.031 & \NA     & 34.710 & 1.647  & 261.586          & \NA     \\
        \NameDomain{turbulence}{HPC}               & 0.441               & 0.145             & 0.063           & 0.489 & 0.990 & 1.825          & 0.145 & 0.027 & 0.034 & 73.444  & 30.805 & 1.473  & 235.055          & 66.419  \\
        \NameDomain{wave}{HPC}               & 0.717               & 0.217             & 0.112           & 1.104 & 1.272 & 4.683          & 0.139 & 0.034 & 0.033 & 103.520 & 30.712 & 1.460  & 256.988          & 75.999  \\
        \NameDomain{hurricane}{HPC}               & 0.504               & 0.174             & \NA             & 0.495 & 1.419 & 1.488          & \NA   & 0.046 & 0.028 & 93.979  & 30.424 & 1.809  & 243.778          & 67.586  \\
        % \hline\hline
        \cline{2-15}
        \NameDomain{citytemp}{TS}                & 0.152               & 0.109             & 0.053           & 0.141 & 1.118 & 0.741          & 0.142 & 0.045 & 0.027 & 88.142  & 28.176 & 0.475  & 144.801          & 56.984  \\
        \NameDomain{ts-gas}{TS}                & 0.642               & 0.186             & 0.071           & 0.922 & 1.403 & 3.080          & 0.118 & 0.033 & 0.034 & 90.527  & 30.670 & 2.034  & 248.964          & 81.300  \\
        \NameDomain{phone-gyro}{TS}                & 0.611               & 0.173             & 0.075           & 0.869 & 1.281 & 0.967          & 0.297 & 0.040 & 0.037 & 71.971  & 28.664 & 1.694  & 253.557          & 261.696 \\
        \NameDomain{wesad-chest}{TS}                & 0.672               & 0.256             & 0.079           & 1.043 & 2.052 & 0.966          & 0.301 & 0.053 & 0.029 & 73.710  & 27.887 & 3.221  & 253.955          & 261.480 \\
        \NameDomain{jane-street}{TS}                & 0.654               & 0.157             & 0.075           & 1.153 & 0.955 & 1.984          & 0.367 & 0.040 & 0.032 & \NA     & 29.331 & 1.616  & 259.426          & 81.645  \\
        \NameDomain{nyc-taxi}{TS}                & 0.797               & 0.129             & 0.081           & 1.198 & 1.414 & 1.027          & 0.241 & 0.049 & 0.030 & \NA     & 28.211 & 3.170  & 219.355          & 262.811 \\
        \NameDomain{gas-price}{TS}                & 0.831               & 0.165             & 0.082           & 1.239 & 1.265 & 1.042          & 0.309 & 0.036 & 0.044 & \NA     & 28.389 & 3.881  & 257.897          & 263.055 \\
        \NameDomain{solar-wind}{TS}                & 0.643               & 0.165             & 0.061           & 0.916 & 1.158 & 1.016          & 0.117 & 0.043 & 0.027 & 76.956  & 29.637 & 1.064  & 254.227          & 260.294 \\
        % \hline\hline
        \cline{2-15}
        \NameDomain{acs-wht}{OBS}               & 0.655               & 0.178             & 0.068           & 0.897 & 1.278 & 3.084          & 0.128 & 0.045 & 0.036 & 119.537 & 30.141 & 1.847  & 236.824          & 79.646  \\
        \NameDomain{hdr-night}{OBS}               & 0.663               & 0.206             & 0.058           & 1.406 & 2.246 & 2.715          & 0.117 & 0.044 & 0.026 & 88.921  & 30.728 & 2.346  & 214.969          & 72.254  \\
        \NameDomain{hdr-lalermo}{OBS}               & 0.733               & 0.215             & 0.068           & 1.755 & 2.525 & 3.208          & 0.191 & 0.051 & 0.027 & \NA     & 30.792 & 2.784  & 244.880          & 74.755  \\
        \NameDomain{hst-wfc3-uvis}{OBS}               & 0.616               & 0.198             & 0.076           & 0.611 & 1.384 & 2.469          & 0.137 & 0.061 & 0.044 & 84.679  & 29.523 & 2.187  & 213.712          & 94.281  \\
        \NameDomain{hst-wfc3-ir}{OBS}               & 0.291               & 0.165             & 0.075           & 0.252 & 1.240 & 1.014          & 0.133 & 0.043 & 0.043 & 92.819  & 29.022 & 2.164  & 148.971          & 77.675  \\
        \NameDomain{spitzer-irac}{OBS}               & 0.617               & 0.189             & 0.066           & 0.720 & 1.213 & 2.564          & 0.137 & 0.049 & 0.039 & 78.357  & 30.574 & 1.916  & 223.544          & 80.831  \\
        \NameDomain{g24-78-usb}{OBS}               & 0.663               & 0.161             & 0.060           & 1.152 & 1.013 & 2.404          & 0.201 & 0.040 & 0.035 & \NA     & 30.912 & 1.548  & 260.501          & 69.587  \\
        \NameDomain{jws-mirimage}{OBS}               & 0.595               & 0.153             & 0.062           & 0.680 & 1.281 & 1.796          & 0.123 & 0.031 & 0.033 & 105.544 & 30.027 & 1.625  & 250.369          & 80.921  \\
        % \hline\hline
        \cline{2-15}
        \NameDomain{tpcH-order}{DB}                & 0.526               & 0.159             & 0.073           & 0.623 & 1.328 & 2.090          & 0.327 & 0.044 & 0.029 & 109.567 & 27.772 & 1.519  & 244.177          & 77.773  \\
        \NameDomain{tpcxBB-store}{DB}                & 0.685               & 0.180             & 0.075           & 1.285 & 1.478 & 1.030          & 0.256 & 0.045 & 0.035 & \NA     & 27.413 & 2.810  & 257.849          & 262.928 \\
        \NameDomain{tpcxBB-web}{DB}                & 0.672               & 0.177             & 0.074           & 1.322 & 1.367 & 1.033          & 0.241 & 0.043 & 0.034 & \NA     & 28.818 & 2.661  & 261.673          & 263.328 \\
        \NameDomain{tpcH-lineitem}{DB}                & 0.687               & 0.128             & 0.065           & 1.202 & 1.238 & 1.029          & 0.113 & 0.039 & 0.030 & \NA     & 30.470 & 2.092  & 259.098          & 262.053 \\
        \NameDomain{tpcDS-catalog}{DB}                & 0.555               & 0.139             & 0.057           & 0.664 & 1.161 & 0.912          & 0.132 & 0.044 & 0.028 & 72.592  & 30.446 & 1.578  & 249.906          & 255.454 \\
        \NameDomain{tpcDS-store}{DB}                & 0.617               & 0.147             & 0.057           & 0.822 & 1.171 & 0.969          & 0.130 & 0.047 & 0.028 & 75.454  & 30.982 & 1.788  & 253.698          & 259.086 \\
        \NameDomain{tpcDS-web}{DB}                & 0.470               & 0.136             & 0.057           & \NA   & \NA   & 0.792          & 0.133 & 0.044 & 0.028 & 69.331  & 30.370 & 1.465  & 239.637          & 247.518 \\
        % \hline\hline
        \cline{2-15}
        \textbf{arithmetic mean} & 0.564               & 0.181             & 0.079           & 0.923 & 1.407 & \textbf{2.192} & 0.202 & 0.047 & 0.034 & 87.778  & 29.595 & 2.716  & \textbf{240.280} & 142.635 \\
        \cline{2-15}
        % \multicolumn{1}{c}{}\\
        % \multicolumn{1}{c}{}\\
                \rowfont{\bfseries}
        \multicolumn{1}{r}{\begin{tabular}{@{}r@{}}\fontfamily{ugq}\selectfont %\normalsize 
        DECOMPRESSION
        % \\domain \& name
        \end{tabular}}   & 
        % {domain} & 
        \TableHead{pFPC}    & 
        \TableHead{SPDP}    & 
        \TableHead{fpzip}   & 
        \TableHead{\TwoLineTabTitle{shf+}{LZ4}}   & 
        \TableHead{\TwoLineTabTitle{shf+}{zstd}}  & 
        \TableHead{\TwoLineTabTitle{ndzip}{-CPU}} & 
        \TableHead{BUFF}     & 
        \TableHead{Gorilla}  & 
        \TableHead{Chimp}    & 
        \TableHead{GFC}      & 
        \TableHead{MPC}      & 
        \TableHead{\TwoLineTabTitle{nv::}{LZ4}}   & 
        \TableHead{\TwoLineTabTitle{nv::}{btcmp}} & 
        \TableHead{\TwoLineTabTitle{ndzip}{-GPU}} 
        \\
        \cline{2-15}
        \textbf{arithmetic mean} & 0.351               & 0.178             & 0.074           & 1.181 & 1.328 & \textbf{1.636} & 0.254 & 0.146 & 0.175 & 99.258 & 28.513 & 53.352 & 122.483 & \textbf{159.312} \\
        \cline{2-15}
        % \bottomrule
\end{tabu}

==> tables/comp_time.tex <==
\begin{tabular}{@{} lrrrrrrrrrrrrrr @{}}
	\toprule
	\bfseries Name         & \bfseries pFPC    & \bfseries SPDP     & \bfseries GFC   & \bfseries MPC & \bfseries fpzip
	                       & \bfseries shf+LZ4 & \bfseries shf+zstd
	                       & \bfseries nv+LZ4  & \bfseries nv+btcmp
	                       & \bfseries ndzip-C & \bfseries ndzip-G
	                       & \bfseries BUFF    & \bfseries Gorilla  & \bfseries Chimp
	\\
	\midrule
	\textbf{astro-mhd}     & 671.9             & 1347.3             & X               & 19.3          & 2208.8          & 330.4  & 346.0  & 21.8  & 1.7  & 101.7  & 1287.4 & 1949.5  & 2600.9  & 7187.9
	\\
	\textbf{astro-pt}      & 1618.6            & 3473.3             & X               & 23.6          & 9182.2          & 517.3  & 1604.7 & 8.4   & 3.1  & 383.3  & 1783.1 & 2117.1  & 16824.2 & 21580.4
	\\
	\textbf{citytemp}      & 101.4             & 108.2              & 30.6            & 0.4           & 210.1           & 93.1   & 68.8   & 8.2   & 0.1  & 20.8   & 1125.1 & 79.4    & 85.0    & 284.6
	\\
	\textbf{h3d-temp}      & 368.4             & 565.2              & 218.4           & 3.3           & 1318.4          & 166.8  & 151.5  & 0.9   & 0.6  & 101.5  & 1257.3 & X       & 2090.6  & 3464.5
	\\
	\textbf{hdr-night}     & 138.7             & 154.3              & 56.5            & 0.8           & 336.2           & 147.0  & 89.4   & 48.4  & 0.1  & 23.1   & 1144.1 & X       & 514.6   & 583.0
	\\
	\textbf{miranda3d}     & 12051.0           & 27394.5            & X               & 119.7         & 52937.2         & X      & X      & X     & X    & 1798.8 & 1542.1 & 26527.8 & 31102.4 & 104755.7
	\\
	\textbf{msg-bt}        & 743.8             & 1352.2             & 519.3           & 9.4           & 3731.6          & 251.8  & 457.2  & 166.3 & 35.8 & 188.7  & 1386.1 & 1170.9  & 6103.8  & 7455.2
	\\
	\textbf{num-brain}     & 469.1             & 760.5              & 283.1           & 5.2           & 1958.9          & 213.0  & 275.0  & 87.5  & 0.5  & 91.4   & 1265.5 & 429.9   & 3587.7  & 4319.1
	\\
	\textbf{num-control}   & 543.8             & 1021.3             & 332.7           & 5.9           & 2383.7          & 244.3  & 307.1  & 2.3   & 2.9  & 103.1  & 1318.9 & 369.3   & 3827.2  & 4714.8
	\\
	\textbf{rsim}          & 310.5             & 423.4              & 322.4           & 3.1           & 1351.4          & 105.6  & 207.7  & 57.9  & 0.4  & 40.9   & 1185.1 & 703.5   & 682.6   & 2269.4
	\\
	\textbf{spitzer-irac}  & 513.5             & 880.0              & 174.7           & 5.4           & 2804.4          & 200.5  & 305.9  & 11.3  & 6.9  & 103.3  & 1321.6 & X       & 1197.3  & 3964.2
	\\
	\textbf{tpch-lineitem} & 2917.7            & 7508.0             &                 & 31.2          & 18028.2         & 1038.2 & 5231.0 & 639.4 & 4.2  & 669.9  & 2199.7 & 5518.8  & 6955.2  & 23289.4
	\\
	\textbf{tpch-order}    & 427.4             & 745.3              & 247.5           & 4.4           & 1785.4          & 198.2  & 168.6  & 1.2   & 1.2  & 83.4   & 1252.0 & 441.0   & 2631.1  & 4008.1
	\\
	\textbf{ts-gas}        & 888.1             & 1644.5             & 505.1           & 10.1          & 4447.1          & 258.1  & 641.8  & 217.6 & 1.2  & 157.9  & 1367.3 & 1776.5  & 2227.2  & 7342.2
	\\
	\textbf{turbulence}    & 264.8             & 469.5              & 218.5           & 2.2           & 1152.7          & 109.1  & 164.5  & 0.6   & 0.9  & 47.1   & 1193.6 & 454.1   & 486.5   & 1610.3
	\\
	\textbf{wave}          & 1540.4            & 2444.3             & 1091.7          & 17.6          & 7900.5          & 480.4  & 785.3  & 379.0 & 2.0  & 268.1  & 1632.1 & 2604.5  & 3878.5  & 12923.9
	\\
	\textbf{average}       & 1473.1            & 3143.2             & 33.4            & 16.3          & 6983.6          & 290.2  & 720.3  & 110.1 & 4.1  & 261.5  & 1391.3 & 3395.6  & 5300.3  & 13109.6
	\\
	\bottomrule
\end{tabular}

==> tables/data_access.tex <==
\begin{tabular}{@{}lll rrr r @{}}
        \toprule
        \bfseries Platform & \bfseries Application        & \bfseries Usage      & \bfseries Total reads & \bfseries Total writes & \bfseries R/W ratio  & \bfseries Profile \\
        \midrule
        HPC
                           & \TabHead mpiBLAST            & Protein docking      & 27.7 GB               & 12.8 MB                & $2.1 \times 10^3$    & read-intensive    \\
                           & \TabHead MOM                 & Oceanic model        & 19.5 GB               & 3.2 GB                 & $6.01$               & read-intensive    \\
                           & \TabHead ECOHAM              & Sediment propagation & 0.4 GB                & 9.7 GB                 & $4.2 \times 10^{-2}$ & write-intensive   \\
                           & \TabHead Ray Tracing         & Video processing     & 67.4 GB               & 71.2 GB                & $ 0.94 $             & balanced          \\
        \midrule
        Big Data
                           & \TabHead Sort                & Text processing      & 5.8 GB                & 5.8 GB                 & $ 1.00 $             & balanced          \\
                           & \TabHead Connected Component & Graph processing     & 13.1 GB               & 71.2 MB                & $ 188.40 $           & read-intensive    \\
                           & \TabHead Grep                & Text processing      & 55.8 GB               & 863.8 MB               & $ 64.52 $            & read-intensive    \\
                           & \TabHead Decision Tree       & Machine learning     & 59.1 GB               & 4.7 GB                 & $ 12.57 $            & read-intensive    \\
                           & \TabHead Tokenizer           & Text processing      & 55.8 GB               & 235.7 GB               & $ 0.24 $             & write-intensive   \\
        \bottomrule
\end{tabular}

==> tables/datasets.tex <==
\begin{tabular}{@{} lr *{5}{>{\ttfamily}r} @{}}
       \toprule
       \bfseries Name         & \bfseries Domain & \bfseries Type & \bfseries Size(\#Bytes) & \bfseries Min Value & \bfseries Max Value & \bfseries \#Nan \\
       \midrule
       \textbf{astro-mhd}     & HPC              & double         & 548,458,560             & 1.000000e+00        & 1.632563e+04        & 0               \\
       \textbf{astro-pt}      & HPC              & double         & 671,088,640             & -6.780964e+00       & 6.788099e+00        & 0               \\
       \textbf{msg-bt}        & HPC              & double         & 266,389,432             & -2.564149e+03       & 1.106146e+10        & 0               \\
       \textbf{num-brain}     & HPC              & double         & 141,840,000             & 0.000000e+00        & 2.828205e+00        & 0               \\
       \textbf{num-control}   & HPC              & double         & 159,504,744             & -6.677789e-01       & 7.120868e-01        & 0               \\
       \textbf{miranda3d}     & HPC              & float          & 4,294,967,296           & 9.992406e-01        & 3.000471e+00        & 0               \\
       \textbf{rsim}          & HPC              & float          & 94,281,728              & 0.000000e+00        & 2.274132e+06        & 0               \\
       \textbf{turbulence}    & HPC              & float          & 67,108,864              & 1.406511e-07        & 1.506619e+02        & 0               \\
       \textbf{wave}          & HPC              & float          & 536,870,912             & -2.783325e-01       & 1.000000e+00        & 0               \\
       \textbf{h3d-temp}      & HPC              & float          & 100,000,000             & nan                 & nan                 & 4767            \\
       \midrule
       \textbf{phone-gyro}    & TS               & double         &                         & -7.9920254          & 14.347641           & 0               \\
       \textbf{wesad-s2}      & TS               & double         & 280,509,376             & -873.67             & 988.08              & 0               \\
       \textbf{citytemp}      & TS               & float          & 11,625,304              & -9.900000e+01       & 1.100000e+02        & 0               \\
       \textbf{ts-gas}        & TS               & float          & 307,452,800             & 0.000000e+00        & 9.091013e+04        & 0               \\
       \textbf{stock-usa}     & TS               & float          &                         &                     &                     &                 \\
       \midrule
       \textbf{hdr-night}     & OBS              & double         & 22,749,792              & nan                 & nan                 & 5201            \\
       \textbf{hdr-hill}      & OBS              & double         & 22,749,792              & nan                 & nan                 & 5201            \\
       \textbf{hst-wfc3-uvis} & OBS              & float          &                         &                     &                     &                 \\
       \textbf{hst-wfc3-ir}   & OBS              & float          &                         &                     &                     &                 \\
       \textbf{hst-acs-wfc}   & OBS              & float          &                         &                     &                     &                 \\
       \textbf{irsa-acs}      & OBS              & float          &                         &                     &                     &                 \\
       \textbf{jws-mirimage}  & OBS              & float          &                         &                     &                     &                 \\
       \textbf{spitzer-irac}  & OBS              & float          & 164,998,080             & nan                 & nan                 & 128132          \\
       \midrule
       \textbf{tpcH-order}    & DB               & double         & 120,000,000             & 8.380500e+02        & 5.588226e+05        & 0               \\
       \textbf{tpcH-lineitem} & DB               & float          & 959,776,816             & 0.000000e+00        & 1.049495e+05        & 0               \\
       \textbf{tpcDS-xxx}     & DB               & float          &                         &                     &                     & 0               \\
       \textbf{tpcI-xxx}      & DB               & float          &                         &                     &                     & 0               \\
       \textbf{tpcxAI-xxx}    & DB               & float          &                         &                     &                     & 0               \\
       \textbf{tpcxBB-xxx}    & DB               & float          &                         &                     &                     & 0               \\
       \textbf{tpcxHS-xxx}    & DB               & float          &                         &                     &                     & 0               \\
       \textbf{tpcxIOT-xxx}   & DB               & float          &                         &                     &                     & 0               \\





       \bottomrule
\end{tabular}

==> tables/decomp_speed.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{@{} rrrrrrrrr|rrrrr @{}}
        % \toprule
        % \bfseries Name           
        % & \bfseries Domain  
        % & 
        \bfseries pFPC      & \bfseries SPDP    & \bfseries fpzip
                                 & \bfseries shf+LZ4 & \bfseries shf+zstd  & \bfseries ndzip-C
                                 & \bfseries BUFF    & \bfseries Gorilla   & \bfseries Chimp
                                 & \bfseries GFC     & \bfseries MPC
                                 & \bfseries nv::LZ4 & \bfseries nv::btcmp
                                 & \bfseries ndzip-G
        \\
        % \midrule
        \hline
        % \textbf{msg-bt}         & HPC & 0.439 & 0.196 & 0.074 & 1.180 & 1.501 & 2.641 & 0.290 & 0.084 & 0.186 & 100.770 & 28.571 & 111.483 & 116.906 & 92.228   \\
        % \textbf{num-brain}      & HPC & 0.394 & 0.184 & 0.076 & 1.191 & 1.203 & 2.425 & 0.392 & 0.101 & 0.169 & 115.876 & 28.552 & 109.119 & 90.415  & 89.196   \\
        % \textbf{num-control}    & HPC & 0.379 & 0.164 & 0.070 & 1.191 & 1.450 & 2.418 & 0.377 & 0.059 & 0.170 & 93.901  & 28.242 & 71.402  & 96.037  & 89.597   \\
        % \textbf{rsim}           & HPC & 0.366 & 0.208 & 0.066 & 1.202 & 1.197 & 1.740 & 0.153 & 0.112 & 0.199 & 95.442  & 28.453 & 15.621  & 67.758  & 112.434  \\
        % \textbf{astro-mhd}      & HPC & 1.734 & 0.374 & 0.239 & 1.194 & 1.351 & 2.011 & 0.332 & 0.738 & 0.420 & \NA     & 28.376 & 79.766  & 189.706 & 212.919  \\
        % \textbf{astro-pt}       & HPC & 0.602 & 0.197 & 0.089 & 1.120 & 1.288 & 2.319 & 0.493 & 0.108 & 0.166 & \NA     & 29.393 & 112.087 & 182.693 & 94.311   \\
        % \textbf{miranda3d}      & HPC & 0.448 & 0.156 & 0.080 & \NA   & \NA   & 2.127 & 0.189 & 0.077 & 0.168 & \NA     & 31.261 & 113.141 & 218.190 & \NA      \\
        % \textbf{turbulence}     & HPC & 0.296 & 0.151 & 0.062 & 1.184 & 1.354 & 1.452 & 0.184 & 0.072 & 0.172 & 89.286  & 28.668 & 74.119  & 54.854  & 94.132   \\
        % \textbf{wave}           & HPC & 0.382 & 0.208 & 0.092 & 1.103 & 1.428 & 2.415 & 0.190 & 0.105 & 0.173 & 103.370 & 28.077 & 80.336  & 169.266 & 98.990   \\	
        % \textbf{hurricane}      & HPC & 0.315 & 0.175 & \NA   & 1.197 & 1.488 & 1.647 & \NA   & 0.107 & 0.160 & 100.142 & 28.520 & 60.228  & 71.982  & 95.033   \\
        % \midrule
        % \textbf{citytemp}       & TS  & 0.134  & 0.108 & 0.055 & 1.301 & 1.968 & 0.602 & 0.148 & 0.162 & 0.140 & 90.224  & 26.591 & 1.570   & 10.425  & 77.335   \\
        % \textbf{ts-gas}         & TS  & 0.389 & 0.189 & 0.066 & 1.196 & 1.201 & 2.332 & 0.154 & 0.088 & 0.166 & 95.669  & 27.735 & 17.840  & 109.882 & 103.859  \\ 
        % \textbf{phone-gyro}     & TS  & 0.347 & 0.177 & 0.071 & 1.184 & 1.394 & 0.991 & 0.378 & 0.061 & 0.185 & 96.058  & 28.603 & 22.671  & 138.906 & 263.914  \\
        % \textbf{wesad-chest}    & TS  & 0.378 & 0.250 & 0.076 & 1.180 & 1.116 & 0.991 & 0.335 & 0.287 & 0.141 & 95.352  & 28.730 & 20.562  & 126.014 & 263.387  \\ 
        % \textbf{jane-street}    & TS  & 0.361 & 0.165 & 0.072 & 1.104 & 1.293 & 1.996 & 0.467 & 0.061 & 0.165 & \NA     & 30.937 & 131.528 & 227.496 & 92.883   \\
        % \textbf{nyc-taxi}       & TS  & 0.423 & 0.121 & 0.076 & 1.158 & 1.213 & 1.030 & 0.314 & 0.255 & 0.135 & \NA     & 28.675 & 21.519  & 111.015 & 263.854  \\ 
        % \textbf{gas-price}      & TS  & 0.517 & 0.160 & 0.082 & 1.159 & 1.093 & 1.026 & 0.374 & 0.095 & 0.220 & \NA     & 28.654 & 30.025  & 196.065 & 263.896  \\ 
        % \textbf{solar-wind}     & TS  & 0.339 & 0.166 & 0.059 & 1.184 & 1.367 & 1.004 & 0.140 & 0.074 & 0.139 & 97.161  & 27.642 & 20.665  & 154.464 & 261.847  \\ 
        % \midrule
        % \textbf{acs-wht}        & OBS & 0.359 & 0.186 & 0.066 & 1.193 & 1.392 & 2.084 & 0.152 & 0.094 & 0.187 & 119.061 & 28.393 & 104.065 & 117.543 & 108.807  \\
        % \textbf{hdr-night}      & OBS & 0.357 & 0.199 & 0.058 & 1.173 & 1.351 & 2.414 & 0.145 & 0.299 & 0.142 & 100.321 & 27.760 & 14.970  & 58.622  & 101.219  \\
        % \textbf{hdr-lalermo}    & OBS & 0.374 & 0.223 & 0.066 & 1.147 & 1.346 & 2.383 & 0.272 & 0.301 & 0.141 & \NA     & 28.155 & 16.410  & 63.797  & 101.756  \\
        % \textbf{hst-wfc3-uvis}  & OBS & 0.394 & 0.188 & 0.070 & 1.194 & 1.223 & 1.723 & 0.166 & 0.114 & 0.228 & 98.489  & 29.159 & 16.322  & 77.103  & 129.732  \\
        % \textbf{hst-wfc3-ir}    & OBS & 0.233 & 0.169 & 0.072 & 1.260 & 1.987 & 0.949 & 0.173 & 0.135 & 0.224 & 94.002  & 27.189 & 6.713   & 19.518  & 108.102  \\
        % \textbf{spitzer-irac}   & OBS & 0.357 & 0.185 & 0.062 & 1.195 & 1.115 & 1.973 & 0.163 & 0.078 & 0.203 & 97.810  & 28.268 & 98.319  & 97.040  & 109.604  \\
        % \textbf{g24-78-usb}     & OBS & 0.345 & 0.160 & 0.058 & 1.190 & 1.151 & 2.023 & 0.264 & 0.058 & 0.180 & \NA     & 29.195 & 112.584 & 216.654 & 95.204   \\
        % \textbf{jws-mirimage}   & OBS & 0.337 & 0.163 & 0.062 & 1.185 & 1.129 & 1.516 & 0.151 & 0.077 & 0.171 & 107.416 & 28.535 & 91.505  & 99.566  & 109.737  \\
        % \midrule
        % \textbf{tpcH-order}     & DB  & 0.314 & 0.167 & 0.071 & 1.189 & 1.660 & 1.882 & 0.437 & 0.088 & 0.134 & 111.872 & 27.998 & 16.798  & 80.658  & 88.768   \\
        % \textbf{tpcxBB-store}   & DB  & 0.362 & 0.181 & 0.072 & 1.123 & 1.191 & 1.034 & 0.315 & 0.128 & 0.162 & \NA     & 27.995 & 22.633  & 182.736 & 263.681  \\
        % \textbf{tpcxBB-web}     & DB  & 0.364 & 0.182 & 0.072 & 1.184 & 1.217 & 1.031 & 0.345 & 0.104 & 0.160 & \NA     & 27.971 & 22.940  & 199.871 & 263.933  \\
        % \textbf{tpcH-lineitem}  & DB  & 0.365 & 0.115 & 0.061 & 1.179 & 1.109 & 1.035 & 0.162 & 0.288 & 0.145 & \NA     & 28.264 & 22.678  & 200.866 & 263.288  \\
        % \textbf{tpcDS-catalog}  & DB  & 0.323 & 0.134 & 0.055 & 1.189 & 1.085 & 0.963 & 0.163 & 0.121 & 0.142 & 95.004  & 28.542 & 46.891  & 101.975 & 262.127  \\
        % \textbf{tpcDS-store}    & DB  & 0.340 & 0.141 & 0.055 & 1.186 & 1.297 & 0.993 & 0.160 & 0.165 & 0.146 & 96.092  & 28.770 & 38.489  & 129.136 & 262.781  \\
        % \textbf{tpcDS-web}      & DB  & 0.296 & 0.133 & 0.055 & \NA   & \NA   & 0.823 & 0.158 & 0.119 & 0.142 & 90.364  & 29.047 & 35.624  & 64.775  & 259.433  \\
        % \hline
        % \textbf{arithmetic mean} & 
        % -                 & 
        0.351               & 0.178             & 0.074           & 1.181 & 1.328 & \textbf{1.636} & 0.254 & 0.146 & 0.175 & 99.258 & 28.513 & 53.352 & 122.483 & \textbf{159.312} \\
        % \bottomrule
\end{tabular}

==> tables/decomp_speed_new.tex <==
% \begin{tabular}{@{} lrrrrrrrrr|rrrrr @{}}
%         \toprule
%         name & pFPC            & SPDP      & fpzip
%              & shf+LZ4         & shf+zstd  & ndzip-C
%              & BUFF            & Gorilla   & Chimp
%              & GFC             & MPC
%              & nv::LZ4         & nv::btcmp
%              & ndzip-G
%         \\
%         \midrule
%         \textbf{arithmetic mean}
%              & \textbf{23.981} & 0.178     & 0.074   & 1.181 & 1.328 & 1.636 & 0.254 & 0.146 & 0.175 & 99.258 & 28.513 & 53.352 & 122.483 & \textbf{159.312} \\
%         \bottomrule
% \end{tabular}


\renewcommand{\arraystretch}{1.2}
\begin{tabu}{@{} l | rrrrr @{}}
    % \toprule
    \hline
    \rowfont{\bfseries}
    CPU (1) & pFPC   & SPDP           & fpzip   & shf+LZ4   & shf+zstd         \\
    GB/s    & 0.351  & 0.178          & 0.074   & 1.181     & 1.328            \\
    % \midrule
    \hline
    \rowfont{\bfseries}
    CPU (2)
            &        & ndzip-C        & BUFF    & Gorilla   & Chimp            \\
    GB/s    &        & \textbf{1.636} & 0.254   & 0.146     & 0.175            \\
    % \midrule
    \hline
    \rowfont{\bfseries\color{RoyalBlue}}
    GPU     & GFC    & MPC            & nv::LZ4 & nv::btcmp & ndzip-G          \\
    \rowfont{\color{RoyalBlue}}
    GB/s    & 99.258 & 28.513         & 53.352  & 122.483   & \textbf{159.312} \\
    \hline
    % \bottomrule
\end{tabu}

==> tables/sc_vs_db.tex <==
\begin{tabular}{@{} >{\bfseries}l ll @{}}
	\toprule
	            & \bf HPC               & \bf TSDB          \\
	\midrule
	algorithm   & prediction-based      & delta-based       \\
	topology    & hyper-cube            & 1-D array         \\
	precision   & high                  & low to medium     \\
	application & scientific simulation & monitoring stream \\
	\bottomrule
\end{tabular}
